An Abstract View on Optimizations in Propositional Frameworks

Search-optimization problems are plentiful in scientific and engineering domains. Artificial intelligence has long contributed to the development of search algorithms and declarative programming languages geared toward solving and modeling search-optimization problems. Automated reasoning and knowledge representation are the subfields of AI that are particularly vested in these developments. Many popular automated reasoning paradigms provide users with languages supporting optimization statements: answer set programming or MaxSAT on minone, to name a few. These paradigms vary significantly in their languages and in the ways they express quality conditions on computed solutions. Here we propose a unifying framework of so-called weight systems that eliminates syntactic distinctions between paradigms and allows us to see essential similarities and differences between optimization statements provided by paradigms. This unifying outlook has significant simplifying and explanatory potential in the studies of optimization and modularity in automated reasoning and knowledge representation. It also supplies researchers with a convenient tool for proving the formal properties of distinct frameworks; bridging these frameworks; and facilitating the development of translational solvers.

==> reviews.tex <==
Reviewer #1: The paper introduces a framework to formalize methods used in MaxSAT and ASP-WC in more general notions.  The author calls this an abstract view on optimization. Therefore, hard and soft constraints are formalized in an abstract system taking modularity and abstraction as key tools for building. The work is an extended version of the JELIA 2021 conference paper "An Abstract View on Optimizations in SAT and ASP".

Unfortunately, I have few, short, but strong concerns:
- While I find the topic quite interesting, I was a bit lost with the overall purpose. The paper introduces some "modular" framework that allows to express both MaxSAT and ASP-WC as well as stating the link between them. However, the actual properties that one aims to express by this are completely missing apart from the semi-formal properties later.  I would have expected a thorough explanation, why one needs a new framework - not just a vague abstract idea that it's good for KRR.  In particular, since there are primarily two frameworks considered (MaxSAT and ASP-WC), a direct reduction might be conceptually much easier. Such a reduction as done in classical complexity theory would link in terms of algorithmic computation providing even technical results on the side. Another way of relating the frameworks could formally be done similar to descriptive complexity, which already aims at richness of logical languages needed to describe problems (link in terms of
expressiveness).
- The Properties 1-4 and Propositions do not seem to be particularly surprising to me - even Proposition 12-14.
- Notation seems to be really heavy, but imprecise and entirely not self-contained. For example, model not formally defined before used, propositional logic and its semantics skipped,
rule operator ← while neither rule nor operator remains undefined, complete and consistent undefined, an assignment function or interpretation, reduct defined operational even though the paper particularly aims for abstract descriptions, logic and formulas mixed (not well worked out why), problems not properly defined, (so far just about the preliminaries), then in propositions statements are not formulated clearly "the equality (19), where Wl is replaced by S, holds then", this continues throughout the paper.
- It is a bit unclear to me what the additional content over the conference version actually is, other than the full proofs. Unfortunately, the author does not state this.


Minors:
- References are largely missing throughout the paper, e.g., the introduction makes plenty of statements that are not justified by references. I would suggest that they are added.
- p2. Why is it the "holy grail"?
- p2. TSP is strangely described. The formulation suggests that one has to enumerate all shortest paths. Doesn't it ask for a/the *shortest* possible route?
- There are some typos in terms of spelling and grammar here and there "Aritificial intelligence", "Let us denotes this w-system", " To illustrate the concept of a reduct" incomplete sentence p4. Grammarly could be of help there.
- Abstract seems to be a bit repetitive and not to the point, might need improvement.
- Definition 12. Is it really necessary to repeat two lines almost exactly?
- Throughout the paper proper motivations, examples, and high-level descriptions are rare and might be improved. In particular, for a journal paper.
- Is there a particular reason that all statements are just propositions and no important statement is emphasized on?
- The paper would benefit if the proofs are moved to the main part.
- Proof Proposition 12: why is the inductive case missing?


Reviewer #2: The article presents weighted abstract modular systems as an abstraction of
search-optimization problems, as expressible by propositional satisfiability
with optimizations (MaxSAT) and answer set programming with weak constraints
(ASP-WC). Such a system consists of a logic module, which imposes hard
constraints and determines models, and weighted conditions, associating
formulas with levels and weights. Then, an optimal model maximizes the sums
of the weights of satisfied formulas, where levels are considered one by one
from higher to lower significance, and min-optimal models minimize these sums.

The article shows that weighted partial MaxSAT and ASP-WC are instances of
weighted abstract modular systems. Some general equivalence transformations are
shown, which include interchangeability of logic modules having the same models,
preservation of (min-)optimal models when weighted conditions yielding the same
sum for all models are eliminated, and convertibility between optimal and
min-optimal models by multiplying all weights with -1. Moreover, transformations
to eliminate either negative or positive weights, map several levels to a single
level by scaling up weights, and turn ASP-WC programs into MaxSAT are developed.
A dedicated section provides proofs for all of the stated theoretical results.

The article is generally well-written and technically sound. What I am reluctant
about is the significance of the presented theoretical results. My impression is
that the role of logic modules is to determine models, where it does not matter
much whether propositional theories or logic programs express hard constraints.
The weighted conditions then represent one objective function per level, and
mathematical transformations of such (pseudo-Boolean) expressions are more or
less well-known, e.g., normalizations similar to the article are discussed in:

Patrik Simons, Ilkka Niemelä, Timo Soininen: Extending and implementing the
stable model semantics. Artif. Intell. 138(1-2): 181-234 (2002)

That is, although the article covers both MaxSAT and ASP-WC and is thus more
general than publications considering either of these fields alone, I struggle
whether there is sufficient novelty.

The following are minor comments concerning the presentation:

- page 1, line 28:
The following sentence in the abstract reads a bit strange in my opinion:
"Recall MaxSAT or answer set programming."

- page 2, lines 11-12:
Consider a well known travelling salesman problem
->
Consider the well known travelling salesman problem

- page 2, lines 25-26:
which translate logic programs into propositional satisfiability (SAT) problem
->
which translate logic programs into the propositional satisfiability (SAT) problem

- page 3, lines 22-23:
advocated by Lierler and Truszczynski [11]
->
advocated by Lierler and Truszczynski [11].

- page 4, lines 45-46:
The following sentence is incomplete:
"To illustrate the concept of a reduct"

- page 5, lines 20-21:
of a considered module in a straight forward manner
->
of a considered module in a straightforward manner

- page 7, line 34:
We call a model l-min-optimal if max is replaced by min in (6)
->
We call a model l-min-optimal if max is replaced by min in (6).

=======================
- page 7, line 45:
Is the "smallest" instead of the "greatest" level l' in \lambda(W) meant in
Lemma 1? (I am unsure whether I got confused and understood Definition 9 wrong.)



Reviewer #3: Part A

CONTENT

Is the paper technically sound? YES

Proof are provided in Section 6 (around 9 pages). They could also go in appendix in my opinion.


Does it show sufficient applicability to AI? YES

MaxSAT and ASP are widely used in AI applications.


Does it place new results in appropriate context with earlier work? NO

Related work is not discussed.


Is the paper sufficiently novel? YES

The proposed formalism was presented at JELIA 2021, and not yet published by any journal.


Is the paper complete? NO

A thorough  discussion of connections with the existing literature is missing.


Does anything need to be added or deleted? YES

Some links with the literature are missing. I would also appreciate a discussion on what should be the role of the properties and propositions given in Section 5; in particular, Propositions 7 and 8 seem of difficult practical use.


Is the result important enough to warrant publication? YES


FORM

Does the abstract adequately reflect the contents? YES

Are the summary and conclusions adequate? YES

Does it contain adequate references to previous work? NO

Does it explain clearly what was done that is new? YES, but

I don't completely agree on some statements.


Does it clearly indicate why this work is important? YES

Is the English satisfactory? YES

Is the presentation otherwise satisfactory? YES

Are there an appropriate number of figures? N/A

Do the figures help clarify the concepts in the paper? N/A


Part B: DETAILED COMMENTS

The paper proposes an abstract framework for logic-based languages with weighted soft constraints. The idea is to view the associated optimization problem at a semantic level, rather than referring to a specific syntax, such as those adopted by MaxSAT and ASP. The framework is formalized, and some properties are shown. MaxSAT and ASP are casted in the framework.

The paper is technically sound in my opinion. Proofs are provided in Section 6, just before concluding the paper. (I am not sure if such proofs should better be given in an appendix. I don't see any particular proving technique here.)


I think that it is good to have a formal framework to highlight similarities between related logic-based languages with weighted soft constraints, but I do not really agree with some statements in the paper. In particular, on page 3, lines 28-35, the author states that

"The formulations of these extensions significantly differ syntactically and semantically from those used in ASP-WC so that the exact link, between ASP-WC and MaxSAT formalisms, required in implementing translational approaches is not obvious. In general, optimizations in different areas of AR (see, for instance, [6, 7, 8, 9, 10, 2]) are studied in separation with no clear articulation of the exact links between the languages expressing optimization criteria and their implementations."

Actually, many algorithms have been shared between MaxSAT, ASP and other formalisms (eg. Abstract Argumentation Frameworks, Constraint Programming and Satisfiability Modulo Theories). The fact that MaxSAT algorithms can be used in ASP is quickly explained in Section 4 of

Mario Alviano, Carmine Dodaro, João Marques-Silva, Francesco Ricca: Optimum stable model search: algorithms and implementation. J. Log. Comput. 30(4): 863-897 (2020)


Also the fact that the framework captures MaxSAT immediately extends to Weighted Propositional Logic (page 11, lines 10-11), because WPL is the formalism associated with the computational problem MaxSAT, and a linear-time Tseitin-like transformation is used to compile the more comfortable syntax of WPL to the more efficiently processable format used by MaxSAT solvers.


Another expected result is that levels are only syntactic sugar (at least for propositional theories). On a first reading, when I reached page 14, lines 41-42 ("In the sequel we often assume level-normal w-systems without loss of generality."), I tought "Why you don't also assume that there is only one level, as done in MaxSAT, where a mixed radix numeral system for the weights is used in case of multilevel optimization?"  Later in the paper, Section 5.2 provides such a mapping. Note that this process is also inverted in some MaxSAT solvers:

Josep Argelich, Inês Lynce, João P. Marques Silva: On Solving Boolean Multilevel Optimization Problems. IJCAI 2009: 393-398


In their current form, it is not clear to me what is the role of the properties provided in Section 5. Some of them are known in MaxSAT and ASP, and the presentation might improve if connections are properly highlighted in the text. For some others (Propositions 7 and 8) some additional explanation should be given, as to me they seem to require an expensive check and therefore cannot be really used to simply problem instances in practice.


All in all, I confirm that it is good to address optimization problems in logic-based languages at a semantic level, and this paper goes in this direction. On the other hand, I think that it should be better to clarify what is the actual contribution by stating already in the introduction the results that are generalized, where they are first shown (in a specific language) or if they are folklore in the MaxSAT and ASP community because implemented in some systems (also pointing to some system descriptions). In the current form, it seems that the results are introduced here for the first time, which is not true and actually muddle readers with a background on the topic. It is more fair to briefly explain that MaxSAT and ASP algorithms take advantage of many structural simplifications, and those simplications can be generalized to the abstract framework. Possibly, in a Related Work section, such links with the literature can be further discussed.

Within this respect, I would like to report that the general purpose approach of ASPRIN was also stated at a semantic level in

Mario Alviano, Javier Romero, Torsten Schaub:
Preference Relations by Approximation. KR 2018: 2-11

In the above paper, knowledge bases are defined as sets of models (similar to the notion of "logic" in Definition 1 of the article under review), and the problem of computing optimal models wrt. some preference relations is addressed. Among the preference relations of ASPRIN (and those considered in the above paper) there are "weight" and "lexico", whose combination gives the preference relation of mainstream ASP (which is also the one considered in the article under review).


Minor suggestions.

P3L14: each city must be visited exactly once (unless there is some assumption on the graph)

P3L18: these >>> those

P5L44-45: there is some typo

P7L36: missing ) in Def.7

P8L20: formally >>> formal

P15L11-12: the equality (19), where W_l is replaced by S, holds  >>> reframe

P15L51: The complement isn't simply sem(\overline{T}) = Int(\sigma_\ell) \setminus sem(T)?

__________________________________________________
In compliance with data protection regulations, you may request that we remove your personal registration details at any time.  (Use the following URL: https://urldefense.com/v3/__https://www.editorialmanager.com/artint/login.asp?a=r__;!!PvXuogZ4sRB2p-tU!Cd9yNauS0aQwOw5j8UBrfoNUHR5LM7aJ9yMRZDVLdK4au0yJD68qVTsFq75IkcG5saLkwkoetO6G_fDANnY$ ). Please contact the publication office if you have any questions.
